Intention-aware policy graphs: answering what, how, and why in opaque agents

Agents are a special kind of AI-based software in that they interact in complex environments and have increased potential for emergent behaviour. Explaining such emergent behaviour is key to deploying trustworthy AI, but the increasing complexity and opaque nature of many agent implementations makes this hard. In this work, we propose a Probabilistic Graphical Model along with a pipeline for designing such model -- by which the behaviour of an agent can be deliberated about -- and for computing a robust numerical value for the intentions the agent has at any moment. We contribute measurements that evaluate the interpretability and reliability of explanations provided, and enables explainability questions such as `what do you want to do now?' (e.g. deliver soup) `how do you plan to do it?' (e.g. returning a plan that considers its skills and the world), and `why would you take this action at this state?' (e.g. explaining how that furthers or hinders its own goals). This model can be constructed by taking partial observations of the agent's actions and world states, and we provide an iterative workflow for increasing the proposed measurements through better design and/or pointing out irrational agent behaviour.

==> figures/cmas_metrics.tex <==

\begin{table}[htb]
    \centering
    \begin{tabular}{c  ll}
        Layout & Mean reward & Std. \\
        \hline
        \textit{simple} & 387.87 & 25.33 \\
        \textit{unident\_s} & 757.71 & 53.03 \\
        \textit{random0} & 395.01 & 54.43 \\
        \textit{random1} & 266.01 & 48.11 \\
        \textit{random3} & 62.5 & 5.00 \\
    \end{tabular}
    \caption{Performance evaluation of trained agent pairs.}
    \label{tab:agent_metrics}
\end{table}

==> figures/marc_metrics.tex <==
simple: Mean Episode Reward = 387.87 and Standard Deviation = 25.33
• unident s: Mean Episode Reward = 757.71 and Standard Deviation = 53.03
• random0 : Mean Episode Reward = 395.01 and Standard Deviation = 54.43
• random1 : Mean Episode Reward = 266.01 and Standard Deviation = 48.11
• random3 : Mean Episode Reward = 62.5 and Standard Deviation = 5.00

==> figures/static_metrics.tex <==

\begin{table}[htb]
    \centering
    \begin{tabular}{ccc|cccc}
    
\multirow{12}*{\simple} &  \multirow{4}*{\cmasone} & 1 & 1.98 & 1.46 & 0.52 & -60.96 \\
& & 2 & 2.15 & 1.41 & 0.74 & -34.66 \\
& & 3 & 2.10 & 1.38 & 0.72 & -25.26 \\
& & 4 & 2.21 & 1.31 & 0.90 & -7.36 \\
\hline
&  \multirow{4}*{\marcone} & 1 & 2.13 & 1.68 & 0.44 &  \\
& & 2 & 2.40 & 1.62 & 0.78 &  \\
& & 3 & 2.47 & 1.50 & 0.98 &  \\
& & 4 & 2.45 & 1.43 & 1.02 &  \\
\hline
&  \multirow{4}*{\cmashuman} & 1 & 3.10 & 1.83 & 1.27 &  \\
& & 2 & 2.90 & 1.71 & 1.20 &  \\
& & 3 & 2.93 & 1.74 & 1.18 &  \\
& & 4 & 2.68 & 1.57 & 1.11 &  \\
\hline
\multirow{12}*{\random0} &  \multirow{4}*{\cmasone} & 1 & 2.17 & 1.70 & 0.48 & -107.99 \\
& & 2 & 2.25 & 1.57 & 0.68 & -107.99 \\
& & 3 & 2.44 & 1.65 & 0.79 & 0.61 \\
& & 4 & 2.40 & 1.49 & 0.91 & 8.61 \\
\hline
&  \multirow{4}*{\marcone} & 1 & 1.54 & 1.03 & 0.50 &  \\
& & 2 & 1.60 & 0.98 & 0.62 &  \\
& & 3 & 1.65 & 0.98 & 0.67 &  \\
& & 4 & 1.68 & 0.93 & 0.75 &  \\
\hline
&  \multirow{4}*{\cmashuman} & 1 & 3.66 & 2.12 & 1.54 &  \\
& & 2 & 3.40 & 1.97 & 1.43 &  \\
& & 3 & 3.55 & 2.05 & 1.50 &  \\
& & 4 & 3.20 & 1.89 & 1.32 &  \\
\hline
\multirow{12}*{\unident_s} &  \multirow{4}*{\cmasone} & 1 & 2.14 & 1.86 & 0.27 & -13.02 \\
& & 2 & 2.26 & 1.76 & 0.49 & -10.82 \\
& & 3 & 2.47 & 1.85 & 0.62 & -13.22 \\
& & 4 & 2.49 & 1.74 & 0.76 & -13.72 \\
&  \multirow{4}*{\marcone} & 1 & 1.37 & 0.90 & 0.47 &  \\
& & 2 & 1.65 & 0.88 & 0.77 &  \\
& & 3 & 1.82 & 0.86 & 0.96 &  \\
& & 4 & 1.89 & 0.84 & 1.06 &  \\
\hline
&  \multirow{4}*{\cmashuman} & 1 & 2.74 & 2.22 & 0.53 &  \\
& & 2 & 2.44 & 1.95 & 0.49 &  \\
& & 3 & 3.05 & 2.18 & 0.87 &  \\
& & 4 & 2.67 & 1.88 & 0.79 &  \\
\hline
\multirow{12}*{\random1} &  \multirow{4}*{\cmasone} & 1 & 2.25 & 1.72 & 0.54 & -72.69 \\
& & 2 & 2.19 & 1.51 & 0.68 & -20.09 \\
& & 3 & 2.39 & 1.56 & 0.84 & -62.99 \\
& & 4 & 2.26 & 1.37 & 0.89 & -8.59 \\
\hline
&  \multirow{4}*{\marcone} & 1 & 1.60 & 1.23 & 0.38 &  \\
& & 2 & 1.58 & 1.12 & 0.46 &  \\
& & 3 & 1.82 & 1.07 & 0.75 &  \\
& & 4 & 1.72 & 1.01 & 0.71 &  \\
\hline
&  \multirow{4}*{\cmashuman} & 1 & 3.29 & 1.99 & 1.30 &  \\
& & 2 & 2.86 & 1.69 & 1.17 &  \\
& & 3 & 2.99 & 1.83 & 1.16 &  \\
& & 4 & 2.59 & 1.55 & 1.04 &  \\
\hline
\multirow{12}*{\random3} &  \multirow{4}*{\cmasone} & 1 & 2.27 & 1.90 & 0.37 & -25.23 \\
& & 2 & 2.31 & 1.81 & 0.50 & -30.13 \\
& & 3 & 2.42 & 1.75 & 0.66 & -14.03 \\
& & 4 & 2.35 & 1.65 & 0.69 & -5.43 \\
\hline
&  \multirow{4}*{\marcone} & 1 & 1.73 & 1.02 & 0.71 &  \\
& & 2 & 1.75 & 0.96 & 0.79 &  \\
& & 3 & 1.92 & 0.98 & 0.94 &  \\
& & 4 & 1.91 & 0.92 & 0.99 &  \\
\hline
&  \multirow{4}*{\cmashuman} & 1 & 3.44 & 2.20 & 1.24 &  \\
& & 2 & 3.14 & 1.99 & 1.15 &  \\
& & 3 & 3.21 & 2.07 & 1.15 &  \\
& & 4 & 2.79 & 1.74 & 1.06 &  \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> figures/texes/intentions_FULL.tex <==

\begin{figure}[htb]
    \centering
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_simple-D11-C0.5.png}
	\label{fig:intention_cmasone_simple_11}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_simple-D14-C0.5.png}
	\label{fig:intention_cmasone_simple_14}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_simple-D21-C0.5.png}
	\label{fig:intention_marcone_simple_21}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_simple-D24-C0.5.png}
	\label{fig:intention_marcone_simple_24}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_simple-D31-C0.5.png}
	\label{fig:intention_cmashuman_simple_31}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_simple-D34-C0.5.png}
	\label{fig:intention_cmashuman_simple_34}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_simple-D41-C0.5.png}
	\label{fig:intention_marctwo_simple_41}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_simple-D44-C0.5.png}
	\label{fig:intention_marctwo_simple_44}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_unident_s-D11-C0.5.png}
	\label{fig:intention_cmasone_unident_s_11}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_unident_s-D14-C0.5.png}
	\label{fig:intention_cmasone_unident_s_14}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_unident_s-D21-C0.5.png}
	\label{fig:intention_marcone_unident_s_21}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_unident_s-D24-C0.5.png}
	\label{fig:intention_marcone_unident_s_24}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_unident_s-D31-C0.5.png}
	\label{fig:intention_cmashuman_unident_s_31}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_unident_s-D34-C0.5.png}
	\label{fig:intention_cmashuman_unident_s_34}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_unident_s-D41-C0.5.png}
	\label{fig:intention_marctwo_unident_s_41}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_unident_s-D44-C0.5.png}
	\label{fig:intention_marctwo_unident_s_44}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_random0-D11-C0.5.png}
	\label{fig:intention_cmasone_random0_11}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_random0-D14-C0.5.png}
	\label{fig:intention_cmasone_random0_14}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_random0-D21-C0.5.png}
	\label{fig:intention_marcone_random0_21}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_random0-D24-C0.5.png}
	\label{fig:intention_marcone_random0_24}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_random0-D31-C0.5.png}
	\label{fig:intention_cmashuman_random0_31}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_random0-D34-C0.5.png}
	\label{fig:intention_cmashuman_random0_34}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_random0-D41-C0.5.png}
	\label{fig:intention_marctwo_random0_41}
\end{subfigure}
\begin{subfigure}[b]{0.245\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/desires_intentions_plots/intentions_random0-D44-C0.5.png}
	\label{fig:intention_marctwo_random0_44}
\end{subfigure}


    \caption{Desire metrics for simple and unident_s environments, for \cmasone and \marcone agents and discretiser 1}
    \label{fig:desire_metrics}
\end{figure}

==> removed_content.tex <==
\begin{comment}
Finally, another optic to evaluate \gls{pg}s can be through evaluating the likelihood of our own observations. To do this, insights from the machine learning community are reused. To build the \gls{pg}, a dataset $\dataset$ of observations is collected. By holding up some episodes from the estimation of $P(s',a|s)$, a validation set $\dataset_v$ is created and one can estimate the fitness of a \gls{pg} representation through computing the (log-) likelihood of the dataset as sum of log-likelihoods of all episodes $E$:

\begin{equation} \label{Eq:log-Likelyhood}
    -\ell(PG;D) = -\sum_{\tikzmarknode{e}{E} \in \dataset_v} log P_G(E) = -\sum_{E \in D_v} log P_{PG}(s_1,a_1 ... a_{t-1},s_{t}) = -\sum_{E \in D_v} \sum_{t \in E} log P_{PG}(s_{t+1},a_t|s_t)
\end{equation}

\begin{comment}

\begin{equation} \label{Eq:log-Likelyhood}
    -\ell(PG;D) = -\sum_{\tikzmarknode{e}{E} \in \dataset_v} log P_G(E) = -\sum_{E \in D_v} log P_{PG}(s_1,a_1 ... a_{t-1},s_{t}) = -\sum_{E \in D_v} \sum_{t \in E} log P_{PG}(s_{t+1},a_t|s_t)
\end{equation}
\begin{tikzpicture}[overlay,remember picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
    % For "X"
    \path (e.south) ++ (0,-0.5em) node[anchor=south east,color=red!67] (scalep){\textbf{Episode}};
    \draw [color=red!87](e.south) |- ([xshift=-0.3ex,color=red]scalep.south west);
\end{tikzpicture}
\end{comment}

This gives an estimator of the performance of \gls{pg} in predicting newer, unseen trajectories, which is linked with the reliability of future explanations (\ie in unseen episodes).  

In practice, the likelihood has a drastic downside, which is that there may be unseen transitions or states in $D_v$, making the likelihood 0. This is very probable for real-world scenarios with a very large amount of variables and proportionally small amount of collected observations. To still allow comparison between \gls{pg}s, a laplace smoothing can be introduced to the probability distribution:

\begin{equation} \label{Eq:a-smoothed-log-Likelyhood}
    \ell^\alpha(PG;D) = \sum_{E \in D} \sum_{t \in E} log \frac{P_{PG}(s_{t+1},a_t|s_t) +\alpha}{1+\alpha|S|}
\end{equation}

Given that $D_v$ may include never-before visited states, $|S|$ should count all possible discretised states, even those not in the \gls{pg}, but we settle for this approximation, since with a small enough $\alpha$ it can be disregarded.

\end{comment}



% IMPORTANT TODOS:
% P(delta s | a) => Action semantics -> Renamed to counterfactuals, lacking do(a) workarounds, moved to downstream paper




% TODO: move below to relwork or background?
\begin{comment}

\gls{pg}s are probabilistic graphical models of the behaviour of agent-environment systems. The key idea is to take already trained agents in an environment and, without taking any assumption on their internal functions (\ie considering them a black box) reduce their interaction with the environment to simple and transparent probability distribution functions that can be interpreted by a human or by understandable algorithms. In order to do so, firstly we reduce states into discrete, explainable representations. In this work we remain agnostic of the particular representation used, only assuming that which state the agent and world are is a discrete choice; and that varying it one gets to different sets of possible states.

% Model P(T) as taking Markov assumption so $P(s_1,a_1, s_2,... s_t) = P(s_1)*\prod_{t=1}^T P(s_{t+1}, a_t|s_t)$. Good properties of these are that one can capture agent behaviour independently of environment $P(a_t|s_t)$, and with informative enough representations of state $s$ one can interpret agent behaviour (\ie why did agent perform action $a$ at state $s_t$? Because it was likely to go to higher valued state $s_{t+1}$, even though it ended up going to $s'_{t+1}$ which was worse but less likely). Attempts done at formalising this Liu et al. focused on qualitative metrics and heuristics.

In this paper, our focus is two-fold. On the one hand, the explainability mechanisms of \gls{pg}s are extended to reliably answer the key question of "\textit{Why} did you take a certain action" via the introduction of desires and intentions and providing more thorough answers to previous \gls{pg} queries~\cite{hayesetal}. 
On the other hand, the methodology for creating and verifying \gls{pg}s is streamlined via adding quantitative evaluation metrics for \gls{pg} reliability and explanation interpretability and also by providing a workflow for producing these explanations to increase the understanding of the agent from a passive point of view, focusing on justifying its behaviour but looking forward to also controlling it, improving it, and discovering new information from it. 

%TODO: integrate better all from below. Perhaps move to methodology?
So far, our own works were centered on evaluating how much does performance of a policy created from the simplified \gls{pg} change wrt the original agent (ie the expected episode reward difference). However, the performance difference does not fully capture everything we could ask of the model: is the difference due to a lack of fidelity in capturing the agents decision? Could there be no difference and still be representing a totally different agent? How closely is the \gls{pg} modelling the agent-world pair? And, how interpretable is the resulting representation in the \gls{pg} model? 

For these purposes, we propose a different set of metrics. These are model agnostic metrics that only consider internal properties of the \gls{pg}, such as which is the expected entropy of a trajectory of T steps performed by the modelled agent. Inspired by this, decomposing entropy in two parts: entropy regarding how well agent behaviour is characterised, and how stochastic is our representation of the environment once an action is taken. The first one measures the fidelity of \gls{pg} to agent behaviour, and the second, the quality to expect from explanations of how actions affect the world's evolution. Finally, for the topic of interpretability, we consider a simple count of nodes and transitions, as the larger the graph gets, the harder it is to interpret it. However, we note that the difficulty of the interpretation is mostly related to each state's internal representation, from which we attempt to remain agnostic in this paper.
\end{comment}


==> semaphor.tex <==


%DEPRECATED OLD SECTION PRESERVED FOR HISTORY
\subsubsection{Traffic light thought experiment}\label{sec:semaphor}

\input{figures/texes/semaphor}


The metrics described in Section~\ref{sec:static_metrics}, as well as the ones used in the literature~\cite{liu thingy, where they use bad entropy} have a considerable weakness, as they assume the uncertainty of action is equally bad in all states or at all times. However, in most real-world scenarios, it is only infrequently when certainty is critical and in most states the action can be liberally chosen. In these cases, the entropy metrics defined above do not work given our lack of context on the criticality of the states. For illustrating this point, we present the \textit{traffic light} environment and agent, as shown in Figure~\ref{fig:semaphor_plot}.

Suppose an environment with three (undiscretised) states, the traffic light is \textit{R}ed, \textit{Y}ellow, \textit{G}reen, in which the agent can take four actions (going up, left, down, or right). The only rewarded transitions are going up on \textit{G}, which gives a positive reward, and going up on \textit{R}, which gives a negative reward. The next state after any action is not affected by the chosen action, to simplify computation. Instead, it has some strong bias toward \textit{Y} or \textit{R} (\eg 50 and 45\%), and a very low probability of going to \textit{G} (eg. 5\%).

Suppose now an agent that interacts with this environment as follows: in the \textit{R} state, it uniformly samples the action between left, down and right (33\%), in \textit{Y} it always goes left, and in \textit{G} it always goes up. This agent has an optimal policy for this environment. This arrangement is visualised in Figure~\ref{fig:semaphor_environment}.

Suppose now two \gls{pg}s, one which distinguishes the \textit{G} state from \textit{Y} and \textit{R} and one which does the same for \textit{R}. Neither will be a perfect surrogate, as all three states had a different probability distribution over actions. The first one can represent an optimal policy, whereas the second cannot (it does not distinguish \textit{Y} from \textit{G}, and the latter is reward-relevant).

However, when computing the agent entropy between these agents, it becomes apparent that $H_a$ is larger (less desirable) for the first case ($0.89$) than for the second ($0.71$). This happens because the relevance of the critical case gets subsumed when considering large numbers. The probability of this happening increases with the size and complexity of the environment, but as has been shown, can happen in toy examples. Although removing from the entropy the weighting of states by their probability (heavily biasing toward infrequent states) or computing entropy on a subset of states found heuristically can reduce the relevance of the problem~\ref{liu}, it can become unreliable if the heuristic is miss-matched for the problem. For example, when choosing as critical states where $H_a$ is low, the \gls{pg} could miss-report explainability in critical states in which action entropy is large, such as the red traffic light in this example. Instead 
